DNN Quantization with Attention

Low-bit quantization of network weights and activations can drastically reduce the memory footprint, complexity, energy consumption and latency of Deep Neural Networks (DNNs). However, low-bit quantization can also cause a considerable drop in accuracy, in particular when we apply it to complex learning tasks or lightweight DNN architectures. In this paper, we propose a training procedure that relaxes the low-bit quantization. We call this procedure \textit{DNN Quantization with Attention} (DQA). The relaxation is achieved by using a learnable linear combination of high, medium and low-bit quantizations. Our learning procedure converges step by step to a low-bit quantization using an attention mechanism with temperature scheduling. In experiments, our approach outperforms other low-bit quantization techniques on various object recognition benchmarks such as CIFAR10, CIFAR100 and ImageNet ILSVRC 2012, achieves almost the same accuracy as a full precision DNN, and considerably reduces the accuracy drop when quantizing lightweight DNN architectures.

==> snippets.tex <==
The idea we propose is to use a selective tensor $\mathbf{A}$ which aims at combining all quantization methods in $\Gamma$ with different scaling factors using a linear interpolation to quantize $\mathbf{W}$. As such, we introduce $\mathbf{A}=\{a_1, a_2, \cdots, a_m\}$ an attention vector containing as many elements as $\Gamma$ and $N$, and in which each value $a_k \in A$ where $1 \leq k \leq m$ is normalized between $0$ and $1$ and represents the importance we give to the quantization method $\Q_k \in \Gamma$ when computing the linear interpolation. At the end of training process, $\mathbf{A}$ becomes binary with only one nonzero value $a_{k^*}$ selecting the quantization method $\Q_{k^*}$ that uses the lowest number of bits $n_{k^*}$ to quantize $\mathbf{W}$ (i.e. $k^* = \arg\min_{k}\{n_k, k=1,2,\cdots,m\}$). %\arg\min_{n \in N}$).  

More precisely, $\mathbf{A}$ is normalized using a softmax function with a temperature $T$. $T$ is decreased smoothly during training process. Note that to force $\mathbf{A}$ to be selective, we first normalize it, so that it has 1 standard deviation (sd), pass it through the softmax function, and finally minimize each value with respect to it importance (the more $n_k$ is higher, the more corresponding value $a_k$ is minimized), thanks to a regularizer we add to the loss function. To introduce such a regularizer, we consider a penalty vector $\mathbf{G}=\{g_1,g_2,\cdots,g_m\}$, and define our new loss function as follows: 

$$
L = L_l +\frac{\lambda}{p}\sum_{k=1}^m g_k \cdot a_k
$$

where $L_l$ is the original loss function, $p$ is the number of parameters in $\mathbf{W}$ of the considered layer and $\lambda$ is the regularization coefficient. Note that both $\lambda$ and temperatur $T$ are used to decide how fast $\mathbf{A}$ is binarized. Consequently, $\lambda$ and $T$ are big and small enough respectively in order to converge to quantization with smaller number of bits, but at the same time not very big and small respectively so the converges is smooth. Regularization term is normalized in order to make its value comparable to $L_l$ and thus find a way to binarize $\mathbf{A}$ with respect to the task to be solved. The increasing function g is used to introduce the importance we give to each $a_k$ according to its corresponding $n_k$. At the end of training process, the selected $Q_k*$ corresponds to the maximum value $a_{k^*}$ in $\mathbf{A}$ and the minimum value $n_{k^*}$ in $\mathbf{N}$. Algorithm~\ref{algo:one} summarizes the training process of one layer and Figure~\ref{fig:my_method} shows an overview the proposed method.

